Face Recognition: Too Bias, or Not Too Bias?

We reveal critical insights into problems of bias in state-of-the-art facial recognition (FR) systems using a novel Balanced Faces In the Wild (BFW) dataset: data balanced for gender and ethnic groups. We show variations in the optimal scoring threshold for face-pairs across different subgroups. Thus, the conventional approach of learning a global threshold for all pairs resulting in performance gaps among subgroups. By learning subgroup-specific thresholds, we not only mitigate problems in performance gaps but also show a notable boost in the overall performance. Furthermore, we do a human evaluation to measure the bias in humans, which supports the hypothesis that such a bias exists in human perception. For the BFW database, source code, and more, visit github.com/visionjo/facerec-bias-bfw.

==> tables/ethnic_splits.tex <==
\scalebox{1}{
     \resizebox{\textwidth}{!}{%
    \begin{tabular}{r c c c c c c c c l}
        \toprule 
        & \multicolumn{2}{c}{Asian (A)} & \multicolumn{2}{c}{Black (B)}  & \multicolumn{2}{c}{Indian (I)}& \multicolumn{2}{c}{White (W)}\\
        \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7}\cmidrule(l){8-9} % spanning less than the full width of the table - you can add (r) or (l) just before the opening curly bracket to shorten the rule on the left or right side
         & Female (AF) & Male (AM) & BF & BM& IF & IM & WF & WM&Aggregated\\ % Column names row
        \midrule

       \# Faces  &  2,500&  2,500& 2,500 & 2,500& 2,500 & 2,500 & 2,500 & 2,500 &20,000 \\ % row 1
        \# Subjects & 100& 100& 100  & 100  & 100  & 100& 100 &100&800  \\ % row 2
        \# Faces / Subject  & 25 & 25    & 25 & 25 & 25  & 25  &  25 & 25 & 25\\ % row 3
        % \midrule
\specialrule{.01em}{.05em}{.05em} 
            \# Positive Pairs &  30,000&  30,000& 30,000 &30,000 & 30,000 &30,000&30,000 & 30,000 &240,000 \\ % row 1
        \# Negative Pairs & 85,135&  85,232& 85,016  & 85,141  & 85,287  & 85,152& 85,223 &85,193&681,379  \\ % row 2
        
        \# Pairs (Total) & 115,135 & 115,232    &115016 &115,141 & 115287  & 115,152  &  115,223& 115193 & 921,379\\ % row 3
        % \midrule
        \specialrule{.01em}{.05em}{.05em} 
        Acc$@t_g$ & 0.876 & 0.944  &0.934 &0.942 &0.922&0.949 &0.916  &0.918&0.925$\pm$0.022 \\ 
        $t_o$ & 0.235 &  0.274 & 0.267&0.254  &0.299 & 0.295& 0.242 &0.222&0.261\\ % row 4
        Acc$@t_o$ & 0.916 &0.964 &0.955 &0.971 &0.933 &0.958 & 0.969 &0.973 & 0.955 $\pm$ 0.018\\ 
        \bottomrule
    \end{tabular}}
    \glsunset{af}
    }
    \glsunset{af}
    \glsunset{am}
    \glsunset{bf}
    \glsunset{bm}
    \glsunset{if}
    \glsunset{im}    
    \glsunset{wf}
    \glsunset{wm}


==> tables/ethnicity_far.tex <==
\begin{center}
\begin{tabular}{l c c c c c}
     \gls{far} & 0.3 & 0.1 & 0.01 & 0.001 & 0.0001\\\midrule
    \multirow{2}{.1mm}{\textbf{\gls{af}}} &0.990 & 0.867 & 0.516 & 0.470 & 0.465\\[-4pt]
        &1.000 & 0.882 & 0.524 & 0.478 & 0.474\\[-1pt]
    \multirow{2}{3mm}{\textbf{\gls{am}}} &0.994 & 0.883 & 0.529 & 0.482 & 0.477\\[-4pt]
        &1.000 & 0.890 & 0.533 & 0.486 & 0.482\\[-1pt]
    \multirow{2}{3mm}{\textbf{\gls{bf}}} &0.991 & 0.870 & 0.524 & 0.479 & 0.473\\[-4pt]
        &1.000 & 0.879 & 0.530 & 0.484 & 0.480\\[-1pt]
    \multirow{2}{3mm}{\textbf{\gls{bm}}} &0.992 & 0.881 & 0.526 & 0.480 & 0.474\\[-4pt]
        &1.000 & 0.891 & 0.532 & 0.485 & 0.480\\[-1pt]
    \multirow{2}{3mm}{\textbf{\gls{if}}} &0.996 & 0.881 & 0.532 & 0.486 & 0.481\\[-4pt]
        &1.000 & 0.884 & 0.534 & 0.488 & 0.484\\[-1pt]
    \multirow{2}{3mm}{\textbf{\gls{im}}} &0.997 & 0.895 & 0.533 & 0.485 & 0.479\\[-4pt]
        &1.000 & 0.898 & 0.535 & 0.486 & 0.481\\[-1pt]
    \multirow{2}{3mm}{\textbf{\gls{wf}}} &0.988 & 0.878 & 0.517 & 0.469 & 0.464\\[-4pt]
        &1.000 & 0.894 & 0.526 & 0.478 & 0.474\\[-1pt]
    \multirow{2}{3mm}{\textbf{\gls{wm}}} &0.989 & 0.896 & 0.527 & 0.476 & 0.470\\[-4pt]
        &1.000 & 0.910 & 0.535 & 0.483 & 0.478\\[-1pt]
    \midrule
    \multirow{2}{3mm}{\textbf{Avg.}} &0.992 & 0.881 & 0.526 & 0.478 & 0.474\\[-4pt]
        &1.000 & 0.891 & 0.531 & 0.483 & 0.479\\[-10pt]
\end{tabular}
\end{center}
